weedNet: Dense Semantic Weed Classification Using Multispectral Images and MAV for Smart Farming

Selective weed treatment is a critical step in autonomous crop management as related to crop health and yield. However, a key challenge is reliable, and accurate weed detection to minimize damage to surrounding plants. In this paper, we present an approach for dense semantic weed classification with multispectral images collected by a micro aerial vehicle (MAV). We use the recently developed encoder-decoder cascaded Convolutional Neural Network (CNN), Segnet, that infers dense semantic classes while allowing any number of input image channels and class balancing with our sugar beet and weed datasets. To obtain training datasets, we established an experimental field with varying herbicide levels resulting in field plots containing only either crop or weed, enabling us to use the Normalized Difference Vegetation Index (NDVI) as a distinguishable feature for automatic ground truth generation. We train 6 models with different numbers of input channels and condition (fine-tune) it to achieve about 0.8 F1-score and 0.78 Area Under the Curve (AUC) classification metrics. For model deployment, an embedded GPU system (Jetson TX2) is tested for MAV integration. Dataset used in this paper is released to support the community and future work.

==> contribs/Discussion.tex <==
% !TEX root = ../weedNet.tex
\section{Discussion and Limitations}
The works presented in this paper only address a point-level segmentation and have not been integrated into the real sweet pepper picking system. We thus do not have measures of the effectiveness/usefulness of the proposed method. This will be assessed shortly after incorporating the proposed system with ROS (e.g., successful picking rate with/without the method). 

Another noticeable limitation of the proposed system is that the trained model yields false positives for other stems and leaves that exhibit similar colour and shape to the peduncle as shown in Fig.~\ref{fig:detection_quatitative_results_with_background}. To overcome this issue, we will make use of context features that take into account the relationship between a sweet pepper and a peduncle. We will calculate a vector between the centroid of a sweet pepper and a point segmented as a peduncle with respect to the gravity vector. With this extra information the supervised learning algorithm will likely be able to determine that peduncles are usually above the centroid at a within a range of distances, improving the false positive rate. The accompanying video demonstration displays the qualitative results in different viewing points\footnoteref{foot:video_data}.
